Explaining Image Classification with Visual Debates

An effective way to obtain different perspectives on any given topic is by conducting a debate, where participants argue for and against the topic. Here, we propose a novel debate framework for understanding and explaining a continuous image classifier's reasoning for making a particular prediction by modeling it as a multiplayer sequential zero-sum debate game. The contrastive nature of our framework encourages players to learn to put forward diverse arguments during the debates, picking up the reasoning trails missed by their opponents and highlighting any uncertainties in the classifier. Specifically, in our proposed setup, players propose arguments, drawn from the classifier's discretized latent knowledge, to support or oppose the classifier's decision. The resulting Visual Debates collect supporting and opposing features from the discretized latent space of the classifier, serving as explanations for the internal reasoning of the classifier towards its predictions. We demonstrate and evaluate (a practical realization of) our Visual Debates on the geometric SHAPE and MNIST datasets and on the high-resolution animal faces (AFHQ) dataset, along standard evaluation metrics for explanations (i.e. faithfulness and completeness) and novel, bespoke metrics for visual debates as explanations (consensus and split ratio).

==> ECAI 2023 Visual Debates/ablation_table.tex <==

\begin{table*}[hbt!]
\centering
\caption{Ablation results with respect to debate length (4, 6 or 10) with mean and variance over three random runs.}
\label{table:noncommittedbehavior}

\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccc|ccc|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}\textsc{Ppty} $\rightarrow$ 
\\ \textsc{Dataset} $\downarrow$\end{tabular}}}  &

\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} \textsc{Feature}  
\\ \textsc{Ext.} $\downarrow$\end{tabular}}} &


\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}\textsc{Codebook}  
\\ \textsc{Sampling} $\downarrow$\end{tabular}}} &

\multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\textsc{Completeness} \end{tabular}}} & 

\multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \textsc{Faithfulness} \end{tabular}}} & 

\multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \textsc{Consensus} \end{tabular}}} & 

\multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} \textsc{Split Ratio} ($Z_R$) \end{tabular}}} \\ 

\cmidrule(l){4-15}
&
&
& {4}                     
& {6}                     
& {10}  

% faithfulness
& {4}                     
& {6}                     
& {10}  

% Reliability
& {4}                     
& {6}                     
& {10}  

% split ratios
& {4}                     
& {6}                     
& {10}                    \\ \cmidrule(r){1-15}

                                                                    
\multirow{6}{*}{{\begin{tabular}[c]{@{}c@{}} 
\\ \textbf{SHAPE}  \\ \end{tabular}}} 


& 
    
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
\textsc{Vanilla} \\ ($0.94 \textcolor{gray}{\pm 0.01}$)  \end{tabular}}} 

& \textsc{Euclidian}

% completeness
& $0.55 \textcolor{gray}{\pm 0.12}$ 
& $0.80 \textcolor{gray}{\pm 0.10}$                             
& $0.85 \textcolor{gray}{\pm 0.02}$ 


% faithfunless
& $0.55 \textcolor{gray}{\pm 0.14}$                             
& $0.79 \textcolor{gray}{\pm 0.07}$                             
& $0.89 \textcolor{gray}{\pm 0.03}$ 

% reliability
& $0.33 \textcolor{gray}{\pm 0.15}$ 
& $0.64 \textcolor{gray}{\pm 0.06}$                             
& $0.78 \textcolor{gray}{\pm 0.01}$ 

% split ratios
& 0.58                               
& 0.60                               
& 0.60                     \\

% ===============================
&
& \textsc{Cosine}


% completeness
& $0.58 \textcolor{gray}{\pm 0.23}$                             
& $0.84 \textcolor{gray}{\pm 0.06}$                             
& $0.82  \textcolor{gray}{\pm 0.01}$    

% faithfulness
& $0.58 \textcolor{gray}{\pm 0.19}$                             
& $0.81 \textcolor{gray}{\pm 0.03}$                             
& $0.88 \textcolor{gray}{\pm 0.02}$ 

% reliability
& $0.34 \textcolor{gray}{\pm 0.16}$ 
& $0.76 \textcolor{gray}{\pm 0.07}$                             
& $0.82 \textcolor{gray}{\pm 0.01}$

% split ratios
& 0.48                               
& 0.56                               
& 0.56                     \\ 


% &
% & \textsc{Gumble}


% % completeness
% & $0.55 \pm 0.12$                               
% & $0.80 \pm 0.10$                                
% & $0.85  \pm 0.02$    

% % faithfulness
% & $0.55 \pm 0.14$                                
% & $0.79 \pm 0.07$                               
% & $0.89 \pm 0.03$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     \\ 
 
\cmidrule(r){2-15}

&
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{ResNet}  \\ ($0.98 \textcolor{gray}{\pm 0.01}$) \end{tabular}}} 

& \textsc{Euclidian}


% completeness
& $0.74 \textcolor{gray}{\pm 0.23}$ 
& $0.83 \textcolor{gray}{\pm 0.14}$                             
& $0.96 \textcolor{gray}{\pm 0.03}$ 


% faithfunless
& $0.76 \textcolor{gray}{\pm 0.12}$                             
& $0.81 \textcolor{gray}{\pm 0.06}$                             
& $0.98 \textcolor{gray}{\pm 0.02}$ 

% reliability
& $0.41 \textcolor{gray}{\pm 0.12}$ 
& $0.58 \textcolor{gray}{\pm 0.05}$                             
& $0.89 \textcolor{gray}{\pm 0.02}$ 

% split ratios
& 0.38                               
& 0.54                               
& 0.58                     \\

% ===============================
&
& \textsc{Cosine}


% completeness
& $0.73 \textcolor{gray}{\pm 0.20}$                             
& $0.81 \textcolor{gray}{\pm 0.08}$                             
& $0.97  \textcolor{gray}{\pm 0.02}$    

% faithfulness
& $0.76 \textcolor{gray}{\pm 0.21}$                             
& $0.83 \textcolor{gray}{\pm 0.04}$                             
& $0.97 \textcolor{gray}{\pm 0.02}$ 

% reliability
& $0.44 \textcolor{gray}{\pm 0.09}$ 
& $0.62 \textcolor{gray}{\pm 0.05}$                             
& $0.91 \textcolor{gray}{\pm 0.01}$

% split ratios
& 0.44                               
& 0.58                               
& 0.58                     \\ 


% &
% & \textsc{Gumble}


% % completeness
% & $0.55 \pm 0.12$                               
% & $0.80 \pm 0.10$                                
% & $0.85  \pm 0.02$    

% % faithfulness
% & $0.55 \pm 0.14$                                
% & $0.79 \pm 0.07$                               
% & $0.89 \pm 0.03$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     \\ 
\cmidrule(r){2-15}

&
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{DenseNet} \\ ($0.96 \textcolor{gray}{\pm 0.02}$)  \end{tabular}}} 

& \textsc{Euclidian}


% completeness
& $0.78 \textcolor{gray}{\pm 0.13}$ 
& $0.89 \textcolor{gray}{\pm 0.04}$                             
& $0.99 \textcolor{gray}{\pm 0.02}$ 


% faithfunless
& $0.81 \textcolor{gray}{\pm 0.07}$                             
& $0.93 \textcolor{gray}{\pm 0.02}$                             
& $0.99 \textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.63 \textcolor{gray}{\pm 0.07}$ 
& $0.68 \textcolor{gray}{\pm 0.05}$                             
& $0.92 \textcolor{gray}{\pm 0.03}$ 

% split ratios
& 0.36                               
& 0.42                               
& 0.60                     \\

% ===============================
&
& \textsc{Cosine}


% completeness
& $0.80 \textcolor{gray}{\pm 0.14}$                             
& $0.91 \textcolor{gray}{\pm 0.03}$                             
& $0.98  \textcolor{gray}{\pm 0.02}$    

% faithfulness
& $0.83 \textcolor{gray}{\pm 0.13}$                             
& $0.94\textcolor{gray}{\pm 0.06}$                             
& $0.98\textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.57 \textcolor{gray}{\pm 0.08}$ 
& $0.65 \textcolor{gray}{\pm 0.06}$                             
& $0.90 \textcolor{gray}{\pm 0.03}$

% split ratios
& 0.38                               
& 0.44                               
& 0.58                     \\

% &
% & \textsc{Gumble}


% % completeness
% & $0.55 \pm 0.12$                               
% & $0.80 \pm 0.10$                                
% & $0.85  \pm 0.02$    

% % faithfulness
% & $0.55 \pm 0.14$                                
% & $0.79 \pm 0.07$                               
% & $0.89 \pm 0.03$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     



\cmidrule(r){1-15}
% =============================
    
\multirow{6}{*}{{\begin{tabular}[c]{@{}c@{}} 
\\ \textbf{MNIST}  \\ \end{tabular}}} 


& 
    
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{Vanilla}  \\ ($0.98 \textcolor{gray}{\pm 0.00}$)\end{tabular}}} 

& \textsc{Euclidian}
                                               

% completeness
& $0.36 \textcolor{gray}{\pm 0.22}$ 
& $0.45 \textcolor{gray}{\pm 0.03}$                             
& $0.73 \textcolor{gray}{\pm 0.01}$ 


% faithfunless
& $0.38 \textcolor{gray}{\pm 0.18}$ 
& $0.49 \textcolor{gray}{\pm 0.01}$                             
& $0.83 \textcolor{gray}{\pm 0.00}$ 

% reliability
& $0.24 \textcolor{gray}{\pm 0.17}$ 
& $0.62 \textcolor{gray}{\pm 0.06}$                             
& $0.74 \textcolor{gray}{\pm 0.04}$ 

% split ratios
& 0.44                               
& 0.45                               
& 0.56     \\

& 
& \textsc{Cosine}
                                               

% completeness
& $0.46 \textcolor{gray}{\pm 0.11}$ 
& $0.58 \textcolor{gray}{\pm 0.06}$                             
& $0.79 \textcolor{gray}{\pm 0.02}$ 


% faithfunless
& $0.53 \textcolor{gray}{\pm 0.08}$                             
& $0.61 \textcolor{gray}{\pm 0.05}$                             
& $0.78 \textcolor{gray}{\pm 0.00}$ 

% reliability
& $0.22 \textcolor{gray}{\pm 0.11}$ 
& $0.58 \textcolor{gray}{\pm 0.02}$                             
& $0.82 \textcolor{gray}{\pm 0.01}$ 


% split ratios
& 0.42                               
& 0.45                               
& 0.55     \\

% &
% & \textsc{Gumble}
                                               

% % completeness
% & $0.56 \pm 0.09$                                
% & $0.60 \pm 0.08$                               
% & $0.74 \pm 0.01$ 


% % faithfunless
% & $0.58 \pm 0.12$                                
% & $0.61 \pm 0.05$                               
% & $0.75 \pm 0.01$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.44                               
% & 0.45                               
% & 0.56     \\ 

\cmidrule(r){2-15}

& 
    
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{ResNet} \\ ($0.99 \textcolor{gray}{\pm 0.00}$) \end{tabular}}} 

& \textsc{Euclidian}
                                               


% completeness
& $0.42 \textcolor{gray}{\pm 0.19}$ 
& $0.46 \textcolor{gray}{\pm 0.08}$                             
& $0.81 \textcolor{gray}{\pm 0.02}$ 


% faithfunless
& $0.45 \textcolor{gray}{\pm 0.13}$ 
& $0.51 \textcolor{gray}{\pm 0.02}$                             
& $0.85 \textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.18 \textcolor{gray}{\pm 0.21}$ 
& $0.57 \textcolor{gray}{\pm 0.09}$                             
& $0.76 \textcolor{gray}{\pm 0.03}$ 

% split ratios
& 0.54                               
& 0.58                               
& 0.61     \\

& 
& \textsc{Cosine}
                                               

% completeness
& $0.38 \textcolor{gray}{\pm 0.22}$ 
& $0.42 \textcolor{gray}{\pm 0.03}$                             
& $0.78 \textcolor{gray}{\pm 0.00}$ 


% faithfunless
& $0.42 \textcolor{gray}{\pm 0.12}$                             
& $0.49 \textcolor{gray}{\pm 0.05}$                             
& $0.81 \textcolor{gray}{\pm 0.00}$ 

% reliability
& $0.21 \textcolor{gray}{\pm 0.09}$ 
& $0.58 \textcolor{gray}{\pm 0.02}$                             
& $0.78 \textcolor{gray}{\pm 0.00}$ 



% split ratios
& 0.43                               
& 0.60                               
& 0.60     \\

% &
% & \textsc{Gumble}
                                               

% % completeness
% & $0.56 \pm 0.09$                                
% & $0.60 \pm 0.08$                               
% & $0.74 \pm 0.01$ 


% % faithfunless
% & $0.58 \pm 0.12$                                
% & $0.61 \pm 0.05$                               
% & $0.75 \pm 0.01$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.44                               
% & 0.45                               
% & 0.56     \\ 

\cmidrule(r){2-15}

& 
    
\multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{DenseNet} \\ ($0.99 \textcolor{gray}{\pm 0.00}$) \end{tabular}}} 

& \textsc{Euclidian}                                          

% completeness
& $0.38 \textcolor{gray}{\pm 0.09}$ 
& $0.54 \textcolor{gray}{\pm 0.05}$                             
& $0.83 \textcolor{gray}{\pm 0.00}$ 


% faithfunless
& $0.41 \textcolor{gray}{\pm 0.15}$ 
& $0.55 \textcolor{gray}{\pm 0.06}$                             
& $0.86 \textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.31 \textcolor{gray}{\pm 0.21}$ 
& $0.76 \textcolor{gray}{\pm 0.04}$                             
& $0.87 \textcolor{gray}{\pm 0.02}$ 

% split ratios
& 0.39                               
& 0.49                               
& 0.51     \\

& 
& \textsc{Cosine}
                                               

& $0.42 \textcolor{gray}{\pm 0.18}$ 
& $0.56 \textcolor{gray}{\pm 0.04}$                             
& $0.77 \textcolor{gray}{\pm 0.01}$ 


% faithfunless
& $0.41 \textcolor{gray}{\pm 0.19}$ 
& $0.56 \textcolor{gray}{\pm 0.09}$                             
& $0.84 \textcolor{gray}{\pm 0.03}$ 

% reliability
& $0.28 \textcolor{gray}{\pm 0.23}$ 
& $0.74 \textcolor{gray}{\pm 0.06}$                             
& $0.85 \textcolor{gray}{\pm 0.01}$ 


% split ratios
& 0.44                               
& 0.49                               
& 0.51     \\

% &
% & \textsc{Gumble}
                                               

% % completeness
% & $0.56 \pm 0.09$                                
% & $0.60 \pm 0.08$                               
% & $0.74 \pm 0.01$ 


% % faithfunless
% & $0.58 \pm 0.12$                                
% & $0.61 \pm 0.05$                               
% & $0.75 \pm 0.01$ 

% % reliability
% &
% &
% &

% % split ratios
% & 0.44                               
% & 0.45                               
% & 0.56     \\ 

\cmidrule(r){1-15}
% ===============================


\multirow{6}{*}{{\begin{tabular}[c]{@{}c@{}} 
\\ \textbf{AFHQ}  \\ \end{tabular}}} 

&
 \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{Vanilla} \\ $(0.96 \textcolor{gray}{\pm 0.02})$ \end{tabular}}} 

& \textsc{Euclidian}
  
% completeness
& $0.81 \textcolor{gray}{\pm 0.09}$                            
& $0.86 \textcolor{gray}{\pm 0.06}$                              
& $0.89 \textcolor{gray}{\pm 0.05}$

% faithfulness
& $0.89 \textcolor{gray}{\pm 0.02}$                             
& $0.91 \textcolor{gray}{\pm 0.04}$                              
& $0.94 \textcolor{gray}{\pm 0.03}$

% reliability
& $0.35 \textcolor{gray}{\pm 0.11}$
& $0.43 \textcolor{gray}{\pm 0.08}$  
& $0.82 \textcolor{gray}{\pm 0.04}$  

% split ratios
& 0.39                               
& 0.44                               
& 0.50                     \\ 

% ===============================
&
& \textsc{Cosine}

% completeness
& $0.31 \textcolor{gray}{\pm 0.10}$                              
& $0.68 \textcolor{gray}{\pm 0.02}$                                
& $0.77 \textcolor{gray}{\pm 0.02}$    

% faithfulness
& $0.33 \textcolor{gray}{\pm 0.09}$                                
& $0.71 \textcolor{gray}{\pm 0.04}$                               
& $0.82 \textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.38 \textcolor{gray}{\pm 0.11}$
& $0.63 \textcolor{gray}{\pm 0.05}$
& $0.76 \textcolor{gray}{\pm 0.02}$

% split ratios
& 0.44                               
& 0.48                               
& 0.49                     \\

% &
% & \textsc{Gumble}

% % completeness
% & $0.31 \textcolor{gray}{\pm 0.13}$
% & $0.58 \textcolor{gray}{\pm 0.02}$                                
% & $0.63 \textcolor{gray}{\pm 0.04}$    

% % faithfulness
% & $0.34 \textcolor{gray}{\pm 0.09}$                                
% & $0.67 \textcolor{gray}{\pm 0.02}$                               
% & $0.68 \textcolor{gray}{\pm 0.04}$ 

% % reliability
% & $0.32 \textcolor{gray}{\pm 0.05}$
% & $0.34 \textcolor{gray}{\pm 0.06}$
% & $0.42 \textcolor{gray}{\pm 0.02}$

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     \\ 

\cmidrule(r){2-15}
% =============================

&
 \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{ResNet}  \\ ($0.98 \textcolor{gray}{\pm 0.01}$ \end{tabular}}} 

& \textsc{Euclidian}
  
% completeness
& $0.76 \textcolor{gray}{\pm 0.06}$                            
& $0.84 \textcolor{gray}{\pm 0.01}$                              
& $0.91 \textcolor{gray}{\pm 0.01}$

% faithfulness
& $0.81 \textcolor{gray}{\pm 0.07}$                             
& $0.90 \textcolor{gray}{\pm 0.02}$                              
& $0.97 \textcolor{gray}{\pm 0.00}$

% reliability
& $0.30 \textcolor{gray}{\pm 0.08}$
& $0.69 \textcolor{gray}{\pm 0.03}$
& $0.93 \textcolor{gray}{\pm 0.02}$

% split ratios
& 0.38                               
& 0.41                               
& 0.43                     \\ 

% ===============================
&
& \textsc{Cosine}

% completeness
& $0.58 \textcolor{gray}{\pm 0.08}$                               
& $0.72 \textcolor{gray}{\pm 0.03}$                                
& $0.88 \textcolor{gray}{\pm 0.00}$    

% faithfulness
& $0.64 \textcolor{gray}{\pm 0.06}$                                
& $0.75 \textcolor{gray}{\pm 0.02}$                               
& $0.92 \textcolor{gray}{\pm 0.01}$ 

% reliability
& $0.40 \textcolor{gray}{\pm 0.18}$
& $0.63 \textcolor{gray}{\pm 0.08}$
& $0.72 \textcolor{gray}{\pm 0.07}$


% split ratios
& 0.40                               
& 0.42                               
& 0.41                     \\

% &
% & \textsc{Gumble}

% % completeness
% & $0.33 \textcolor{gray}{\pm 0.08}$                               
% & $0.44 \textcolor{gray}{\pm 0.02}$                                
% & $0.91 \textcolor{gray}{\pm 0.01}$    

% % faithfulness
% & $0.37 \textcolor{gray}{\pm 0.06}$                                
% & $0.59 \textcolor{gray}{\pm 0.00}$                               
% & $0.93 \textcolor{gray}{\pm 0.01}$ 

% % reliability
% & $0.38 \textcolor{gray}{\pm 0.14}$
% & $0.48 \textcolor{gray}{\pm 0.01}$
% & $0.54 \textcolor{gray}{\pm 0.03}$

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     \\ 

\cmidrule(r){2-15}

&
 \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}} 
 \textsc{DenseNet} \\ $(0.65 \textcolor{gray}{\pm 0.08})$ \end{tabular}}} 

& \textsc{Euclidian}
  
% completeness
& $0.49 \textcolor{gray}{\pm 0.12}$                            
& $0.54 \textcolor{gray}{\pm 0.11}$                              
& $0.58 \textcolor{gray}{\pm 0.08}$

% faithfulness
& $0.54 \textcolor{gray}{\pm 0.12}$                             
& $0.60 \textcolor{gray}{\pm 0.06}$                              
& $0.62 \textcolor{gray}{\pm 0.02}$

% reliability
& $0.31 \textcolor{gray}{\pm 0.11}$
& $0.40 \textcolor{gray}{\pm 0.09}$
& $0.56 \textcolor{gray}{\pm 0.04}$

% split ratios
& 0.60                               
& 0.63                               
& 0.68                     \\ 

% ===============================
&
& \textsc{Cosine}

% completeness
& $0.41 \textcolor{gray}{\pm 0.23}$                               
& $0.40 \textcolor{gray}{\pm 0.08}$                                
& $0.65 \textcolor{gray}{\pm 0.02}$    

% faithfulness
& $0.43 \textcolor{gray}{\pm 0.13}$                                
& $0.43 \textcolor{gray}{\pm 0.04}$                               
& $0.65 \textcolor{gray}{\pm 0.03}$ 

% reliability
& $0.33 \textcolor{gray}{\pm 0.16}$
& $0.48 \textcolor{gray}{\pm 0.02}$
& $0.60 \textcolor{gray}{\pm 0.00}$

% split ratios
& 0.72                               
& 0.72                               
& 0.77                     \\

% &
% & \textsc{Gumble}

% % completeness
% & $0.41 \textcolor{gray}{\pm 0.11}$                               
% & $0.51 \textcolor{gray}{\pm 0.06}$                                
% & $0.52 \textcolor{gray}{\pm 0.06}$

% % faithfulness
% & $0.46 \textcolor{gray}{\pm 0.14}$                                
% & $0.55 \textcolor{gray}{\pm 0.03}$                               
% & $0.57 \textcolor{gray}{\pm 0.04}$ 

% % reliability
% & $0.31 \textcolor{gray}{\pm 0.13}$
% & $0.40 \textcolor{gray}{\pm 0.00}$
% & $0.53 \textcolor{gray}{\pm 0.01}$

% % split ratios
% & 0.58                               
% & 0.60                               
% & 0.60                     \\ 
\bottomrule
\end{tabular}
}
\end{table*}
